Paranatural Category Theory

We establish and advocate for a novel branch of category theory, centered around strong dinatural transformations (herein known as "paranatural transformations"). Paranatural transformations generalize natural transformations to mixed-variant difunctors, but, unlike other such generalizations, are composable and exceptionally well-behaved. We define the category of difunctors and paranatural transformations, prove a novel "diYoneda Lemma" for this category, and explore some of the category-theoretic implications. We also develop three compelling uses for paranatural category theory: parametric polymorphism, impredicative encodings of (co)inductive types, and difunctor models of type theory. Paranatural transformations capture the essence of parametricity, with their "paranaturality condition" coinciding exactly with the "free theorem" of the corresponding polymorphic type; the paranatural analogue of the (co)end calculus provides an elegant and general framework for reasoning about initial algebras, terminal coalgebras, bisimulations, and representation independence; and "diYoneda reasoning" facilitates the lifting of Grothendieck universes into difunctor models of type theory. We develop these topics and propose further avenues of research.

==> agda/Paranatural/DiYonedaTranspose.tex <==
\subsection{Paranatural.DiYonedaTranspose}

\begin{code}[hide]%
\>[0]\AgdaSymbol{\{-\#}\AgdaSpace{}%
\AgdaKeyword{OPTIONS}\AgdaSpace{}%
\AgdaPragma{--without-K}\AgdaSpace{}%
\AgdaPragma{--safe}\AgdaSpace{}%
\AgdaSymbol{\#-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Paranatural.DiYonedaTranspose}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Level}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Categories.Category}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\AgdaSpace{}%
\AgdaSymbol{as}\AgdaSpace{}%
\AgdaModule{≡}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≡\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Categories.Morphism}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{GenDifunctor.Core}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Paranatural.Core}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{private}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{variable}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaGeneralizable{ℓ}\AgdaSpace{}%
\AgdaGeneralizable{e}\AgdaSpace{}%
\AgdaGeneralizable{o′}\AgdaSpace{}%
\AgdaGeneralizable{ℓ′}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPostulate{Level}\<%
\\
%
\>[4]\AgdaGeneralizable{C}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{Category}\AgdaSpace{}%
\AgdaGeneralizable{o}\AgdaSpace{}%
\AgdaGeneralizable{ℓ}\AgdaSpace{}%
\AgdaGeneralizable{e}\<%
\end{code}
\begin{formal}[\cref{defn:DiYonedaTranspose}]\label{agda:DiYonedaTranspose}\ 

\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{--\ record\ ParanaturalTransformation\ }\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \{C\ :\ Category\ o\ ℓ\ e\}\ (D\ E\ :\ GenDifunctor\ C\ o′\ ℓ′)\ }\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ :\ Set\ (o\ ⊔\ ℓ\ ⊔\ e\ ⊔\ o′\ ⊔\ ℓ′)\ where}\<%
\\
\>[0]\AgdaComment{--\ \ \ eta-equality}\<%
\\
\>[0]\AgdaComment{--\ \ \ private}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ module\ C\ =\ Category\ C}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ module\ D\ =\ GenDifunctor\ D}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ module\ E\ =\ GenDifunctor\ E}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ open\ Categories.Morphism\ C}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ \ \ field}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ α\ \ :\ ∀\ I\ →\ D.Objᴰ\ I\ →\ E.Objᴰ\ I\ }\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ preserve-hom\ :\ ∀\ \{I\ J\}\ (j\ :\ C\ [\ I\ ,\ J\ ])\ \{x\}\ \{y\}\ →\ }\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ \ \ \ \ D.Homᴰ\ j\ x\ y\ →\ E.Homᴰ\ j\ (α\ I\ x)\ (α\ J\ y)}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ preserve-coe\ :\ ∀\ \{I\ J\}\ (I≅J\ :\ I\ ≅\ J)\ \{x\ :\ D.Objᴰ\ I\}\ →\ }\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ \ \ \ \ α\ J\ (D.coe\ I≅J\ x)\ ≡\ E.coe\ I≅J\ (α\ I\ x)}\<%
\end{code}
\end{formal}

==> content/defn/DiYonedaTranspose.tex <==
%% content/defn/DiYonedaTranspose.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% June 2026
%%
Given a generalized difunctor $\mb E$ over $\C$, define the generalized difunctor $\widetilde{\mb E}$
\begin{itemize}
\item an element $\varphi$ of $\widetilde{\mb E}_I$ is a family of functions $$ \varphi_K \colon I\cong K \to \mb E_K$$ for each object $K$ of $\C$ such that, for $j\colon I\cong J$ and $k\colon J\cong K$, $$ \coe[\mb E](k,\varphi_J\;j) = \varphi_K\;(k\circ j)$$
\item $(\varphi,\psi)$ is in $\widetilde{\mb E}_j$ iff $$ (\varphi_I\;\iden_I,\psi_J\;\iden_J) \in \mb E_j$$
\item for $j\colon I\cong J$ and $\varphi\colon\widetilde{\mb E}_I$, define $\coe[\sim](j,\varphi)\colon\widetilde{\mb E}_J$ by $$ (\coe[\sim](j,\varphi))_K\;(k\colon J\cong K) \dEqual \varphi_K(k\circ j) $$
\end{itemize}


==> content/defn/DinaturalTransformation.tex <==
%% content/defn/DinaturalTransformation.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% June 2026
%%
Given difunctors $\Gamma, \Delta\colon\C\op\times\C\to\SET$, a \textbf{dinatural transformation} $\alpha\colon \Gamma\tod\Delta$ consists of a family of maps $$ \alpha_I\colon \Gamma(I,I) \to \Delta(I,I) $$ for each object $I$ of $\C$ such that, for all morphisms $j\colon\C\:[I,J]$ and elements $w\colon\Gamma(J,I)$, $$ \Delta(I,j)\;(\alpha_I\;(\Gamma(j,I)\;w)) = \Delta(j,J)\;(\alpha_J\;(\Gamma(J,j)\;w)), $$ i.e. $\Delta(I,j)\circ\alpha_I\circ\Gamma(j,I) = \Delta(j,J)\circ\alpha_J\circ\Gamma(J,j)$.


==> content/defn/GenDifunctor.tex <==
%% content/defn/GenDifunctor.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% June 2026
%%

A \textbf{generalized difunctor} $\mb D$ over a category $\mb C$ is a faithful displayed category over $\C$, equipped with an operation $$ \coe[\mb D]\colon I \cong J \to \mb D_I \to \mb D_J $$ such that $\coe[\mb D](\iden,x)=x$, $\coe[\mb D](k\circ j,x)=\coe[\mb D](k,\coe[\mb D](j,x))$ and $$ (x,\coe[\mb D](j,x)) \in \mb D_j. $$


==> content/defn/InitialAlgebraGenDifunctor.tex <==
%% content/defn/InitialAlgebraGenDifunctor.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% June 2026
%%
An \textbf{initial algebra} for a generalized difunctor $\mb D$ over $\mb C$ consists of an object $\mu_{\mb D}$ of $\C$ and an element $\inn_{\mb D}\colon\mb D_{\mu_{\mb D}}$ such that, for each $I$ and each $x\colon\mb D_I$, there exists a unique morphism $\rec\;x\colon\C\:[\mu_{\mb D},I]$ such that $$ (\inn_{\mb D},x) \in \mb D_{\rec\;x}. $$


==> content/defn/ParanaturalTransformation.tex <==
%% content/defn/ParanaturalTransformation.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% June 2026
%%

Given generalized difunctors $\mb D,\mb E$  over $\mb C$, a \textbf{paranatural transformation} from $\mb D$ to $\mb E$ is a family of functions $\alpha_I\colon\mb D_I \to \mb E_I$ for each object $I$ of $\mb C$ such that
\begin{itemize}
    \item ($\alpha$ preserves morphisms): for each morphism $j\colon\mb C\:[I,J]$, if $(x,y)\in \mb D_j$, then $(\alpha_I\;x,\alpha_J\;y)\in\mb E_j$
    \item ($\alpha$ preserves $\coe$): $\alpha_J(\coe[\mb D](j,x)) = \coe[\mb E](j,\alpha_I\;x)$ for every $j\colon I\cong J$.
\end{itemize}



==> content/defn/StrongDinaturalTransformation.tex <==
%% content/defn/StrongDinaturalTransformation.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% June 2026
%%
Given difunctors $\Gamma,\Delta\colon\C\op\times\C\to\SET$, a \textbf{strong dinatural transformation} $\alpha\colon\Gamma\tos\Delta$ consists of a family of maps $$ \alpha_I \colon \Gamma(I,I) \to \Delta(I,I) $$ for each object $I$ of $\C$ such that, for all morphisms $j\colon\C\:[I,J]$ and elements $x\colon \Gamma(I,I)$ and $y\colon\Gamma(J,J)$,
\begin{equation} \label{tag:EQstrongDinat}
\Gamma(I,j)\;x = \Gamma(j,J)\;y \qquad\text{implies}\qquad \Delta(I,j)\;(\alpha_I\;x) = \Delta(j,J)\;(\alpha_J\;y).
\end{equation}


==> content/defn/TotalCat.tex <==
%% content/defn/TotalCat.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% June 2026
%%
Given a generalized difunctor $\mb D$ over $\C$, define the \textbf{total category} $\Sigma\mb D$ of $\mb D$ to be the category whose
\begin{itemize}
\item objects are pairs $(I,x)$ where $x\colon\mb D_I$
\item morphisms $(I,x)\to(J,y)$ are $\C$-morphisms $j\colon\C\:[I,J]$ such that $(x,y)\in\mb D_j$.
\end{itemize}


==> content/defn/coe-difunctor.tex <==
%% content/defn/coe-difunctor.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% June 2026
%%

For $x\colon\Gamma(I,I)$ and a $\C$-isomorphism $j\colon I\cong J$, write $$ \coe[\Gamma](j,x) \dEqual \Gamma(j\inv,j)\;x $$



==> content/defn/faithfulDisplayedCategory.tex <==
%% content/defn/faithful displayed category.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% June 2026
%%

A \textbf{faithful displayed category} $\mb D$ over a category $\C$ consists of
\begin{itemize}
\item  \textit{a family of sets:} for each object $I$ of $\C$, a set $\mb D_I$
\item  \textit{a heterogeneous preorder:} for each morphism $j\colon\C\:[I,J]$, a relation $\mb D_j\subseteq \mb D_I \times \mb D_J$ such that :
    \begin{itemize}
    \item $(x,x)\in \mb D_\iden$, for all $x$,
    \item if $(x,y)\in \mb D_j$ and $(y,z)\in\mb D_k$, then $(x,z)\in\mb D_{k\circ j}$, for all $x,y,z,j,k$.
    \end{itemize}
\end{itemize}


==> content/defn/faithful_displayed_category.tex <==
%% content/defn/faithful displayed category.tex
%%
%% By Jacob Neumann (jacobneu.com)
%% June 2026
%%

A \textbf{faithful displayed category} $\mb D$ over a category $\C$ consists of
\begin{itemize}
\item  \textit{a family of sets:} for each object $I$ of $\C$, a set $\mb D_I$
\item  \textit{a heterogeneous preorder:} for each morphism $j\colon\C\:[I,J]$, a relation $\mb D_j\subseteq \mb D_I \times \mb D_J$ such that :
    \begin{itemize}
    \item $(x,x)\in \mb D_\iden$, for all $x$,
    \item if $(x,y)\in \mb D_j$ and $(y,z)\in\mb D_k$, then $(x,z)\in\mb D_{k\circ j}$, for all $x,y,z,j,k$.
    \end{itemize}
\end{itemize}

